Spectral asymptotics on sequences of elliptically degenerating Riemann surfaces

This is the second in a series of two articles where we study various aspects of the spectral theory associated to families of hyperbolic Riemann surfaces obtained through elliptic degeneration. In the first article, we investigate the asymptotics of the trace of the heat kernel both near zero and infinity and we show the convergence of small eigenvalues and corresponding eigenfunctions. Having obtained necessary bounds for the trace, this second article presents the behavior of several spectral invariants. Some of these invariants, such as the Selberg zeta function and the spectral counting functions associated to small eigenvalues below 1/4, converge to their respective counterparts on the limiting surface. Other spectral invariants, such as the spectral zeta function and the logarithm of the determinant of the Laplacian diverge. In these latter cases, we identify diverging terms and remove their contributions, thus regularizing convergence of these spectral invariants. Our study is motivated by a result from \cite{He 83}, which D. Hejhal attributes to A. Selberg, proving spectral accumulation for the family of Hecke triangle groups. In this article, we obtain a quantitative result to Selberg's remark.

==> psbox.tex <==
%% Every macro likes a little privacy...
\catcode`\@=11


                  %% -------------------------- %%


%%
%% Trying to tame the variety of \special commands for Postscript: the
%% universal internal command \PSspeci@l##1##2 takes ##1 to be the
%% filename and ##2 to be the integer scale factor*1000 (as for usual
%% TeX \scale commands)
%

\def\psfortextures{%     For TeXtures on the Macintosh
\def\PSspeci@l##1##2{%
\special{illustration ##1\space scaled ##2}}}

                          %% ----------- %%

\def\psfordvips{%      For DVIPS converter on VAX, UNIX and PC's
\def\PSspeci@l##1##2{%
\d@my=0.1bp \d@mx=\drawingwd \divide\d@mx by\d@my%
\special{PSfile=##1\space llx=\psllx\space lly=\pslly\space%
urx=\psurx\space ury=\psury\space rwi=\number\d@mx}}}

                          %% ----------- %%

%%
%% Correspond parfaitement a la doc OzTeX.
%% 
\def\psforoztex{%        For the OzTeX shareware on the Macintosh
\def\PSspeci@l##1##2{%
\special{##1 \space
      ##2 1000 div dup scale
      \putsp@ce{\number-\psllx} \putsp@ce{\number-\pslly} translate}}}
\def\putsp@ce#1{#1 }

                          %% ----------- %%

\def\psonlyboxes{%     Draft-like behaviour if none of the others works
\def\PSspeci@l##1##2{%
\at{0cm}{0cm}{\boxit{\vbox to\drawinght
  {\vss
  \hbox to\drawingwd{\at{0cm}{0cm}{\hbox{(##1)}}\hss}
  }}}}}


                  %% -------------------------- %%


%%
%% \ReadPSize{PSfilename} reads the dimensions of a PostScript drawing
%% and stores it in \drawinght(wd)
%%
\newdimen\drawinght\newdimen\drawingwd
\newdimen\psxoffset\newdimen\psyoffset
\newbox\drawingBox

\newread\epsffilein    % file to \read
\newif\ifepsffileok    % continue looking for the bounding box?
\newif\ifepsfbbfound   % success?
\newif\ifepsfverbose   % report what you're making?
\newdimen\epsfxsize    % horizontal size after scaling
\newdimen\epsfysize    % vertical size after scaling
\newdimen\epsftsize    % horizontal size before scaling
\newdimen\epsfrsize    % vertical size before scaling
\newdimen\epsftmp      % register for arithmetic manipulation
\newdimen\pspoints     % conversion factor
%%
\pspoints=1bp          % Adobe points are `big'
\epsfxsize=0pt         % Default value, means `use natural size'
\epsfysize=0pt         % ditto


\def\ReadPSize#1{
\edef\PSfilename{#1}
\global\def\epsfllx{72}
\global\def\epsflly{72}
\global\def\epsfurx{540}
\global\def\epsfury{720}
%%
%%   The first thing we need to do is to open the
%%   PostScript file, if possible.
%%
\openin\epsffilein=#1
\ifeof\epsffilein\errmessage{I couldn't open #1, will ignore it}\else
%%
%%   Okay, we got it. Now we'll scan lines until we find one that doesn't
%%   start with %. We're looking for the bounding box comment.
%%
   {\epsffileoktrue \chardef\other=12
    \def\do##1{\catcode`##1=\other}\dospecials \catcode`\ =10
    \loop
       \read\epsffilein to \epsffileline
       \ifeof\epsffilein\epsffileokfalse\else
%%
%%   We check to see if the first character is a % sign;
%%   if not, we stop reading (unless the line was entirely blank);
%%   if so, we look further and stop only if the line begins with
%%   `%%BoundingBox:'.
%%
          \expandafter\epsfaux\epsffileline:. \\%
       \fi
   \ifepsffileok\repeat
   \ifepsfbbfound\else
    \ifepsfverbose\message{No bounding box comment in #1; using defaults}\fi\fi
   }\closein\epsffilein\fi
\def\psllx{\epsfllx}\def\pslly{\epsflly}%
\def\psurx{\epsfurx}\def\psury{\epsfury}%
%% Units related by crazy factors as bp/pt=72.27/72 should be BANNED!
\drawinght=\epsfury bp%
\advance\drawinght by-\epsflly bp%
\drawingwd=\epsfurx bp%
\advance\drawingwd by-\epsfllx bp%
}

%%
%%   We still need to define the tricky \epsfaux macro. This requires
%%   a couple of magic constants for comparison purposes.
%%
{\catcode`\%=12 \global\let\epsfpercent=%\global\def\epsfbblit{%BoundingBox}}%
%%
%%   So we're ready to check for `%BoundingBox:' and to grab the
%%   values if they are found.
%%
%% \long\def\epsfaux#1#2:#3\\{\ifx#1\epsfpercent
%%    \def\testit{#2}\ifx\testit\epsfbblit
%%       \epsfgrab #3 . . . \\%
%%       \epsffileokfalse
%%       \global\epsfbbfoundtrue
%%    \fi\else\ifx#1\par\else\epsffileokfalse\fi\fi}%
\long\def\epsfaux#1#2:#3\\{\ifx#1\epsfpercent
   \def\testit{#2}\ifx\testit\epsfbblit
      \epsfgrab #3 @ @ @ \\%
      \epsffileokfalse
      \global\epsfbbfoundtrue
   \fi\else\ifx#1\par\else\epsffileokfalse\fi\fi}%

%%
%%   Here we grab the values and stuff them in the appropriate definitions.
%%
%% \def\epsfgrab #1 #2 #3 #4 #5\\{%
%%    \global\def\epsfllx{#1}\ifx\epsfllx\empty
%%       \epsfgrab #2 #3 #4 #5 .\\\else
%%    \global\def\epsflly{#2}%
%%    \global\def\epsfurx{#3}\global\def\epsfury{#4}\fi}%
\def\epsfgrab #1 #2 #3 #4 #5\\{%
   \global\def\epsfllx{#1}\ifx\epsfllx\empty
      \epsfgrab #2 #3 #4 #5 @\\\else
   \global\def\epsflly{#2}%
   \global\def\epsfurx{#3}\global\def\epsfury{#4}\fi}%


                  %% -------------------------- %%


%%
%% \psboxto(xdim;ydim){psfilename}: you specify the dimensions and
%%    TeX uniformly scales to fit the largest one. If xdim=0pt, the
%%    scale is fully determined by ydim and vice versa.
%%    Notice: psboxes are a real vboxes; couldn't take hbox otherwise all
%%    indentation and all cr's would be interpreted as spaces (hugh!).
%%
\newcount\xscale \newcount\yscale \newdimen\pscm\pscm=1cm
\newdimen\d@mx \newdimen\d@my
\let\ps@nnotation=\relax
\def\psboxto(#1;#2)#3{\vbox{
   \catcode`\:=12
   \ReadPSize{#3}
   \divide\drawingwd by 1000
   \divide\drawinght by 1000
   \d@mx=#1
   \ifdim\d@mx=0pt\xscale=1000
         \else \xscale=\d@mx \divide \xscale by \drawingwd\fi
   \d@my=#2
   \ifdim\d@my=0pt\yscale=1000
         \else \yscale=\d@my \divide \yscale by \drawinght\fi
   \ifnum\yscale=1000
         \else\ifnum\xscale=1000\xscale=\yscale
                    \else\ifnum\yscale<\xscale\xscale=\yscale\fi
              \fi
   \fi
   \divide \psxoffset by 1000\multiply\psxoffset by \xscale
   \divide \psyoffset by 1000\multiply\psyoffset by \xscale
   \global\divide\pscm by 1000
   \global\multiply\pscm by\xscale
   \multiply\drawingwd by\xscale \multiply\drawinght by\xscale
   \ifdim\d@mx=0pt\d@mx=\drawingwd\fi
   \ifdim\d@my=0pt\d@my=\drawinght\fi
\message{[#3\space [BoundingBox\string:\space\epsfllx\space\epsflly\space\epsfurx\space\epsfury]}%
\message{[scaled\space\the\xscale\string:\space\the\drawingwd\space x \the\drawinght]]}%
 \hbox to\d@mx{\hss\vbox to\d@my{\vss
   \global\setbox\drawingBox=\hbox to 0pt{\kern\psxoffset\vbox to 0pt{
      \kern-\psyoffset
      \PSspeci@l{\PSfilename}{\the\xscale}
      \vss}\hss\ps@nnotation}
   \global\ht\drawingBox=\the\drawinght
   \global\wd\drawingBox=\the\drawingwd
   \baselineskip=0pt
   \copy\drawingBox
 \vss}\hss}
  \global\psxoffset=0pt
  \global\psyoffset=0pt% These are local to one figure
  \global\pscm=1cm
  \global\drawingwd=\drawingwd
  \global\drawinght=\drawinght
}}


                  %% -------------------------- %%

%%
%% \psboxscaled{scalefactor*1000}{PSfilename} allows to bypass the
%%   rounding errors of TeX integer divisions for situations where the
%%   TeX box should fit the original BoundingBox with a precision better
%%   than 1/1000.
%%
\def\psboxscaled#1#2{\vbox{
  \catcode`\:=12
  \ReadPSize{#2}
  \xscale=#1
  \divide\drawingwd by 1000\multiply\drawingwd by\xscale
  \divide\drawinght by 1000\multiply\drawinght by\xscale
  \divide \psxoffset by 1000\multiply\psxoffset by \xscale
  \divide \psyoffset by 1000\multiply\psyoffset by \xscale
  \global\divide\pscm by 1000
  \global\multiply\pscm by\xscale
\message{[#2\space [BoundingBox\string:\space\epsfllx\space\epsflly\space\epsfurx\space\epsfury]}%
\message{[scaled\space\the\xscale\string:\space\the\drawingwd\space x \the\drawinght]]}%
  \global\setbox\drawingBox=\hbox to 0pt{\kern\psxoffset\vbox to 0pt{
     \kern-\psyoffset
     \PSspeci@l{\PSfilename}{\the\xscale}
     \vss}\hss\ps@nnotation}
  \global\ht\drawingBox=\the\drawinght
  \global\wd\drawingBox=\the\drawingwd
  \baselineskip=0pt
  \copy\drawingBox
  \global\psxoffset=0pt
  \global\psyoffset=0pt% These are local to one figure
  \global\pscm=1cm
  \global\drawingwd=\drawingwd
  \global\drawinght=\drawinght
}}


                  %% -------------------------- %%

%%
%%  \psbox{PSfilename} makes a TeX box having the minimal size to
%%      enclose the picture
\def\psbox#1{\psboxscaled{1000}{#1}}


                  %% -------------------------- %%

%%
%%  Annotations & Captions etc...
%%
%% \centinsert{anybox} is just a centered \midinsert, but is included as
%% people barely use the original inserts from TeX.
%%
\def\centinsert#1{\midinsert\line{\hss#1\hss}\endinsert}
\def\psannotate#1#2{\def\ps@nnotation{#2\global\let\ps@nnotation=\relax}#1}
\def\pscaption#1#2{\vbox{
   \setbox\drawingBox=#1
   \copy\drawingBox
   \vskip\baselineskip
   \vbox{\hsize=\wd\drawingBox\setbox0=\hbox{#2}
     \ifdim\wd0>\hsize
       \noindent\unhbox0\tolerance=5000
    \else\centerline{\box0}
    \fi
}}}


                  %% -------------------------- %%


%%
%% \at{#1}{#2}{#3} puts #3 at #1-higher and #2-right of the current
%%    position without moving it (to be used in annotations).
%%
\def\at#1#2#3{\setbox0=\hbox{#3}\ht0=0pt\dp0=0pt
  \rlap{\kern#1\vbox to0pt{\kern-#2\box0\vss}}}


                  %% -------------------------- %%


%%
%% \gridfill(ht;wd) makes a 1cm*1cm grid of ht by wd whose lower-left
%%   corner is the current point
%%
\newdimen\gridht \newdimen\gridwd
\def\gridfill(#1;#2){
  \setbox0=\hbox to 1\pscm
  {\vrule height1\pscm width.4pt\leaders\hrule\hfill}
  \gridht=#1
  \divide\gridht by \ht0
  \multiply\gridht by \ht0
  \advance \gridht by \ht0
  \gridwd=#2
  \divide\gridwd by \wd0
  \multiply\gridwd by \wd0
  \advance \gridwd by \wd0
  \vbox to \gridht{\leaders\hbox to\gridwd{\leaders\box0\hfill}\vfill}}


                  %% -------------------------- %%


%%
%% Useful to measure where to put annotations
%%
\def\fillinggrid{\at{0cm}{0cm}{\vbox{\gridfill(\drawinght;\drawingwd)}}}


                  %% -------------------------- %%


%%
%% \frameit{\thick}{\skip}{\anybox}
%%    draws with thickness \thick a box around \anybox, leaving \skip of
%%    blank around it. eg \frameit{0.5pt}{1pt}{\hbox{hello}}
%% \boxit{\anybox} is a shortcut.
%%
\def\frameit#1#2#3{\hbox{\vrule width#1\vbox{
  \hrule height#1\vskip#2\hbox{\hskip#2\vbox{#3}\hskip#2}%
        \vskip#2\hrule height#1}\vrule width#1}}
\def\boxit#1{\frameit{0.4pt}{0pt}{#1}}


                  %% -------------------------- %%


\catcode`\@=12 % cs containing @ are unreachable
%\catcode`\@=\active % cs containing @ are unreachable
 


